Occlusion Resilient 3D Human Pose Estimation

Occlusions remain one of the key challenges in 3D body pose estimation from single-camera video sequences. Temporal consistency has been extensively used to mitigate their impact but the existing algorithms in the literature do not explicitly model them. Here, we apply this by representing the deforming body as a spatio-temporal graph. We then introduce a refinement network that performs graph convolutions over this graph to output 3D poses. To ensure robustness to occlusions, we train this network with a set of binary masks that we use to disable some of the edges as in drop-out techniques. In effect, we simulate the fact that some joints can be hidden for periods of time and train the network to be immune to that. We demonstrate the effectiveness of this approach compared to state-of-the-art techniques that infer poses from single-camera sequences.

==> figures/tex-figs/fig_graphs.tex <==
\begin{figure}
    \centering
    \includegraphics[width=5cm,keepaspectratio]{figures/pngs/graph-new.png}
    \caption{\small A diagrammatic illustration of $\mathcal{G}$ used to model the spatial-temporal dependencies between different joints present in a human body. Each joint is represented with a different solid color. The temporal edges (colored) connect the same joints across between consecutive frames, while the spatial edges represent the natural skeletal structure of the human body. Please note that we are not showing all the joints so as to avoid any clutter in the representation of $\mathcal{G}$.}
    \label{fig:spatial-temporal-graph}
\end{figure}

% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={left,top},capbesidewidth=2.5cm}}]{figure}[\FBwidth]
% {\caption{\small A diagrammatic illustration of $\mathcal{G}$ used to model the spatial-temporal dependencies between different joints present in a human body. Each joint is represented with a different solid color. The temporal edges (colored) connect the same joints across between consecutive frames, while the spatial edges represent the natural skeletal structure of the human body. Please note that we are not showing all the joints so as to avoid any clutter in the representation of $\mathcal{G}$.}\label{fig:spatial-temporal-graph}}
% {\includegraphics[width=5cm]{figures/pngs/graph-new.png}}
% \end{figure}


% \begin{figure}
% \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
% {\caption{\small A diagrammatic illustration of $\mathcal{G}$ used to model the spatial-temporal dependencies between different joints present in a human body. Each joint is represented with a different solid color. The temporal edges (colored) connect the same joints across between consecutive frames, while the spatial edges represent the natural skeletal structure of the human body. Please note that we are not showing all the joints so as to avoid any clutter in the representation of $\mathcal{G}$.}\label{fig:spatial-temporal-graph}}
% {\includegraphics[width=5cm,keepaspectratio]{figures/pngs/graph-new.png}}
% \end{figure}

==> tables/table_mask_choices.tex <==
\begin{table}[]
\caption{A study of generating structured masks using~\cite{Durasov21a} against the random dropping of the features with a certain rate $\tau$.}
\label{tab:mask_choices}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\toprule
Method & \multicolumn{5}{c|}{$\tau$}   & Ours \\
\midrule
       & 0.0 & 0.1 & 0.2 & 0.3 & 0.5 &      \\
\midrule
MPJPE  &   &     &     &     &     &      \\
% \midrule
NMPJPE &   &     &     &     &     &      \\
% \midrule
PMPJPE &   &     &     &     &     &   \\  
\bottomrule
\end{tabular}
\end{table}

==> tables/table_num_masks.tex <==

\begin{table*}[t]
\centering
\caption{A comparative study of generating different number of structured masks using~\cite{Durasov21a}.%Our proposed method with 32 masks is shown in \textbf{bold}.
}
\label{tab:num_masks}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
$\textrm{N}_{\textrm{M}}$ & 0 & 1 & 2 & 4 & 8 & 12 & 16 & 24 & 32 & 40 & 48 & 64 \\ \hline
\textbf{MPJPE}~$\downarrow$ & 60.2  & 60.5 & 60.7 & 60.5 & 60.1 & 59.7 & 59.1 & 58.5 & \textbf{58.2} & 58.2 & 58.3 & 58.3 \\ \hline
\end{tabular}
\end{table*}

==> tex_files/limitations.tex <==

\subsection{Limitations}

As discussed in Section~\ref{sec:fullResults}, a limitation of our approach is that it relies on a pre-trained joint 2D detector~\cite{roy22a}, whose effectiveness or lack thereof directly impacts our final results. To demonstrate this, we ran an experiment in which we replaced the 2D detections by their ground-truth values and report the results in Table~\ref{tab:h36m_2d_gt}. Unsurprisingly, the metrics are substantially improved. This points toward the fact that the 2D detector should be trained as well and made part of the trainable end-to-end pipeline.  

As also pointed out in Section~\textsection~\ref{sec:fullResults}, we do not enforce any additional weight modulation and sharing practices of~\cite{Zou21,Cai19,Zeng20}, which are key for their good performance in the fully supervised setup. This should be added in future versions of this approach as there is no theoretical obstacle to doing so.
\input{tables/table_2d_gt.tex}

==> tex_files/results-fully.tex <==
%!TEX root = ../main.tex
%!TEX spellcheck = en-US

\input{tables/table_h36m_fully.tex}


\section{Quantitative Results - Fully Supervised} 
\label{sec:fullResults}

We now evaluate our approach on the Human 3.6M and MPI-INF-3DHP datasets in the fully supervised setup: We use {\it all} the  2D and 3D ground truth training annotations that are provided. We report the results for H36M and MPI in Table~\ref{tab:h36m_fully} and~\ref{tab:mpi_fully}. To generate the numbers for~\cite{roy22a}, we used our own implementation. The others are the published ones.

Here, the result are more mixed. Our approach does well overall but the methods of~\cite{Cai19,Iqbal20,Zeng20,Zou21,Chen21} outperform us on some of measures in one of the two datasets. We attribute this to the following differences: First, a pipeline such as that of~\cite{Zou21} relies on a Cascaded Pyramid Network 2D point detector~\cite{Chen18e}, which is reported to be more powerful that the one we use~\cite{roy22a}. We therefore tried using it but this did not change the overall performance of our approach. This suggests that we need to use a more complex deeper backbone network similar to the one used in~\cite{Zou21} to take advantage of it. Second, the method of \cite{Iqbal20} leverages additional datasets in training of their estimation networks, while the approaches of~\cite{Zou21,Cai19,Zeng20} enforce spatial constraints on the weights learned by the GCNN based estimation networks. We do neither of these things, but they could be integrated into our own GCNNs. In short, even though our network operates under more challenging conditions, it still delivers comparable results, which confirms the power of our occlusion-handling scheme. Furthermore, the methods of~\cite{Cai19,Zeng20,Zou21,Chen21} have not been demonstrated in the semi-supervised framework and it is not entirely clear what they would do in this training mode. 

\input{tables/table_mpi_fully.tex}

% Zou21,Cai19,Zeng20

